Performance Analysis of Near-Optimal Energy Buffer Aided Wireless Powered Communication

In this paper, we consider a wireless powered communication system, where an energy harvesting (EH) node harvests energy from a radio frequency (RF) signal broadcasted by an access point (AP) in the downlink (DL). The node stores the harvested energy in an energy buffer and uses the stored energy to transmit data to the AP in the uplink (UL). We investigate two simple online transmission policies for the EH node, namely a best-effort policy and an on-off policy, which do not require knowledge of the EH profile nor channel knowledge. In particular, for both policies, the EH node transmits in each time slot with a constant desired power if sufficient energy is available in its energy buffer. Otherwise, the node transmits with the maximum possible power in the best-effort policy and remains silent in the on-off policy. For both policies, we use the theory of discrete-time continuous-state Markov chains to analyze the limiting distribution of the stored energy for finite- and infinite-size energy buffers. We provide this limiting distribution in closed form for a Nakagami-m fading DL channel and analyze the outage probability for a Nakagami-m fading UL channel. All derived analytical results are not limited to EH via RF WPT but are applicable for any independent and identically distributed EH process, originating from e.g. solar and wind energy. Our results reveal that, for low outage probabilities, the best-effort policy is superior to the on-off policy and the optimal constant UL transmit power of the EH node that minimizes the outage probability is always less than the average harvested power but increases with the capacity of the energy buffer. The opposite behaviour is observed for high outage probabilities. Furthermore, we show that the minimum outage probability of the two proposed policies closely approaches the outage probability of the optimal offline power allocation policy.

==> Arxiv_proof_OO_limiting_dist_Finite_gamma_EH_process.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ARXIV FINITE Finite ON_OFF%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Corollary \ref{coro:limiting_dist_Finite_Nakagami_exact_OO}  (Finite-Size Buffer with On-Off Scheme)}
\label{app:limiting_dist_Finite_Nakagami_exact_OO}
We first derive $g(x)$ for $M<x<K$ in (\ref{eq:g2_OO}) and $\pi(K)$
in (\ref{eq:Pi_K_Nakagami_OO}). Notice that the integral equations of the on-off scheme in (\ref{eq:partb}), (\ref{eq:partc}), and (\ref{eq:partd}) differ from those of the best-effort scheme in (\ref{eq:parta_BE}), (\ref{eq:partb_BE}), and (\ref{eq:partc_BE}), respectively, only in the first term. Hence, when substituting with the pdf and the ccdf of the gamma-distributed EH process in (\ref{eq:partb})-(\ref{eq:partd}), we get (\ref{eq:parta_Nakagami})-(\ref{eq:partc_Nakagami}) with the difference that the first term in the brackets in  (\ref{eq:parta_Nakagami}) and (\ref{eq:partb_Nakagami}) should be replaced by $\int_{u=0}^M(x-u)^{m-1}\e^{\lambda u}g(u)\dd u$, and the first term in the brackets in (\ref{eq:partc_Nakagami}) should be replaced by $\sum_{r=0}^{m-1}\frac{\lambda^r}{r!}\int_{u=0}^{M}\e^{\lambda u} (K-u)^r g(u) \dd u$. Due to this similarity, it follows that the pdf $g(x)$ for the on-off scheme in the ranges $M<x<K-M$, $K-M<x<K$, and $\pi(K)$ are identical to (\ref{eq:parta_Nakagami2}), (\ref{eq:partb_Nakagami2}), and (\ref{eq:partc_Nakagami2}), respectively. The sole difference is in the definition of $I_1(r)$, namely $I_1(r)=\int_{u=0}^M(k-u)^r\e^{\lambda u}g(u)\dd u$ which from (\ref{eq:alpha_r_definition}) would result in different $\alpha_r$.
Now, since the derivations from (\ref{eq:g_integral_eqn_finite_Nakagami2}) to (\ref{eq:gn_Nakagami_step}) are independent of $\alpha_r$, it follows that $g(x)$ for $M<x<K$ and the atom $\pi(K)$ are identical to those of the best-effort scheme. Hence, (\ref{eq:g2_OO}) and (\ref{eq:Pi_K_Nakagami_OO}) are identical to (\ref{eq:pdf_Nakagami_m}) and (\ref{eq:Pi_K_Nakagami}), respectively.

It remains to get $g_{l-1}(x)\definedas g(x)$ in the range $0<x<M$ and a non-homogeneous system of equations to get $\alpha_r$, $r=0,\ldots,m-1$.  In the following, we first obtain $g_{l-1}(x)$. Substituting with the pdf of the gamma distributed EH process $f(x)\!=\!\frac{\lambda^m}{\Gamma(m)}x^{m-1}\e^{-\lambda x}$ in (\ref{eq:parta}), we get
\begin{equation}
g_{l-1}(x)=\frac{\lambda^m\e^{-\lambda x}}{(m-1)!}\int\limits_{u=0}^{x}(x-u)^{m-1}\e^{\lambda u}g_{l-1}(u)\dd u+\underbrace{\frac{\lambda^m\e^{-\lambda x}}{(m-1)!}\int\limits_{u=M}^{M+x}(x-u+M)^{m-1}\e^{-\lambda(M-u)}g_{l-2}(u)\dd u}_{T(x)}
\label{eq:g_l_1_OO_step1}
\end{equation}
where $g_{l-2}(x)$ is $g(x)$ in the range $M<x<2M$, i.e., it is given by (\ref{eq:g2_OO}) at $n=l-2$. Eq. (\ref{eq:g_l_1_OO_step1}) is a volterra integral equation of the second kind, whose solution is given by \cite[eq. 2.2-2.31]{polyanin2008handbook}
\begin{equation}
g_{l-1}(x)=T(x)+\underbrace{\int\limits_{u=0}^{x}R(x-u)T(u)\dd u}_{I_R(x)}
\label{eq:g_l_1_OO_step2}
\end{equation}
where 
\begin{equation}
R(x)=\frac{\e^{-\lambda x}}{m}\sum\limits_{k=0}^{m-1}\lambda\e^{\lambda x\cos(\eta_k)}\cos\Big(\eta_k+\lambda x\sin(\eta_k)\Big)
\label{eq:R_x}
\end{equation}
where $\eta_k=\frac{2\pi k}{m}$. Next, we get $T(x)$ defined in (\ref{eq:g_l_1_OO_step1}) by substituting $g_{l-2}(u)$ from (\ref{eq:g2_OO}) at $n=l-2$ in $T(x)$ and solving integrals of the form $\int_{u=M}^{M+x}(x+M-u)^{m-1}(qM-K+u)^d \dd u$ once at $d=(q+1)m-r-1$ and once at $d=qm-1$.  This integral can be solved after replacing $(qM-K+u)^d$ by $\sum_{t=0}^d \binom{d}{t}(u-M)^t((q+1)M-K)^{d-t}$ and using $\int_a^b(b-u)^c(u-a)^t\dd u=\frac{c!t!(b-a)^{c+t+1}}{(c+t+1)!}$ with $a<b$ at $a=M$, $b=M+x$, and $c=m-1$. then $T(x)$ reduces to
\begin{equation}
\begin{aligned}
T(x)&=\e^{-\lambda x}\sum\limits_{r=0}^{m-1}\frac{\alpha_r}{r!}\Biggg[\sum\limits_{q=0}^{l-2}\lambda^{(q+2)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{(q+1)m-r-1}\frac{((q+1)M-K)^{(q+1)m-r-1-t}}{((q+1)m-r-1-t)!(m+t)!}x^{m+t}\\
&-\lambda^r\sum\limits_{q=1}^{l-2}\lambda^{(q+1)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{qm-1}\frac{((q+1)M-K)^{qm-1-t}}{(qm-1-t)!(m+t)!}x^{m+t}\Biggg].
\end{aligned}
\label{eq:T_x}
\end{equation}
Next, we get $I_R(x)$ defined in (\ref{eq:g_l_1_OO_step2}). Using $R(x)$ in (\ref{eq:R_x}) and and $T(x)$ in (\ref{eq:T_x}), $I_R(x)$ can be written as
\begin{equation}
\begin{aligned}
I_R(x)&=\e^{-\lambda x}\sum\limits_{r=0}^{m-1}\frac{\alpha_r}{r!}\Biggg[\sum\limits_{q=0}^{l-2}\lambda^{(q+2)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{(q+1)m-r-1}\frac{((q+1)M-K)^{(q+1)m-r-1-t}}{((q+1)m-r-1-t)!(m+t)!} I_t(x)\\
&-\lambda^r\sum\limits_{q=1}^{l-2}\lambda^{(q+1)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{qm-1}\frac{((q+1)M-K)^{qm-1-t}}{(qm-1-t)!(m+t)!}I_t(x)\Biggg].
\end{aligned}
\label{eq:IR_x}
\end{equation}
where $I_t(x)$ is given by
%\begin{equation}
%\begin{aligned}
%I_t(x)&=\frac{1}{m}\sum\limits_{k=0}^{m-1}\lambda\e^{\lambda x\cos(\eta_k)}\Biggg[\cos\Big(\underbrace{\eta_k+\lambda x\sin(\eta_k)}_{\mu_{k,x}}\Big)\underbrace{\int\limits_{u=0}^{x}u^{m+t}\e^{-\lambda\cos(\eta_k)u}\cos\Big(\lambda\sin(\eta_k)u\Big)\dd u}_{I_{\cos}}\\
%&+\sin\Big(\underbrace{\eta_k+\lambda x\sin(\eta_k)}_{\mu_{k,x}}\Big)\underbrace{\int\limits_{u=0}^{x}u^{m+t}\e^{-\lambda\cos(\eta_k)u}\sin\Big(\lambda\sin(\eta_k)u\Big)\dd u}_{I_{\sin}}\Biggg].
%\end{aligned}
%\label{eq:It_x_step1}
%\end{equation}
\begin{equation}
I_t(x)=\frac{1}{m}\sum\limits_{k=0}^{m-1}\lambda\e^{\lambda x\cos(\eta_k)}\Biggg[\cos(\mu_{k,x})I_{\cos}(x)
+\sin(\mu_{k,x})I_{\sin}(x)\Biggg].
\label{eq:It_x_step1}
\end{equation}
where $\mu_{k,x}=\eta_k+\lambda x\sin(\eta_k)$, $I_{\sin}(x)=\int_{u=0}^{x}u^{m+t}\e^{-\lambda\cos(\eta_k)u}\sin\Big(\lambda\sin(\eta_k)u\Big)\dd u$ and \\$I_{\cos}(x)=\int_{u=0}^{x}u^{m+t}\e^{-\lambda\cos(\eta_k)u}\cos\Big(\lambda\sin(\eta_k)u\Big)\dd u$. 
$I_{\sin}(x)$ and $I_{\cos}(x)$ are solved using \cite[eq. 3.944.1]{table_of_integrals_Ryzhik} and \cite[eq. 3.944.3]{table_of_integrals_Ryzhik}, respectiely as $I_{\cos}=\Re\{I_{\text{complex}}\}$ and $I_{sin}=-\Im\{I_{\text{complex}}\}$, where $I_{\text{complex}}=\Big(\lambda \e^{\J\eta_k}\Big)^{-(m+t+1)}\gamma\Big(m+t+1,\lambda x\e^{\J\eta_k}\Big)$. Substituting back in (\ref{eq:It_x_step1}), $I_t(x)$ reduces to
\begin{equation}
I_t(x)=\frac{1}{m}\sum\limits_{k=0}^{m-1}\lambda\e^{\lambda x\cos(\eta_k)}\Re\{\e^{\J\mu_{k,x}}I_{\text{complex}}\}
=\frac{1}{m}\sum\limits_{k=0}^{m-1}\Re\Big\{(\lambda\e^{\J\eta_k})^{-(m+t)}\e^{\lambda x \e^{\J\eta_k}}\gamma\Big(m+t+1,\lambda x \e^{\J\eta_k}\Big)\Big\}
\label{eq:It_x}
\end{equation}
Substituting $I_{t}(x)$ from (\ref{eq:It_x}) in (\ref{eq:IR_x}) and adding $T(x)$ and $I_R(x)$ in (\ref{eq:T_x}) and (\ref{eq:IR_x}), respectively, $g_{l-1}(x)$ in (\ref{eq:g_l_1_OO_step2}) reduces to (\ref{eq:g1_OO}).\\

Now, it remains to get $\alpha_s$, $s=0,\ldots,m-1$. 
Similar to the best-effort scheme, $\alpha_s$ satisfies (\ref{eq:alpha_r_definition}) where only $I_1(s)$ has a different definition. The remaining terms in $\alpha_s$ can be obtained using the analysis in (\ref{eq:I2_expansion1})-(\ref{eq:I2_expansion3}) with the only difference that in the on-off scheme we assume $K=lM$ with integer $l$, hence in (\ref{eq:I2_expansion1}), the last integral is on $g_{l-2}(x)$ over the limits $M$ to $K-(l-2)M$. Therefore, $I_2(s)$ satisfies (\ref{eq:I2_expansion3}) with the inner summation limits up to $q=l-2$ instead of $q=l-1$. With these considerations, the last two terms in $\alpha_s$ in (\ref{eq:alpha_r_definition}) are given by $I_2(s)+M^s\e^{-\lambda M}\sum\limits_{r=0}^{m-1}\alpha_r\frac{\lambda^r}{r!}=$
\begin{equation}
-\sum\limits_{r=0}^{m-1}\frac{K^s\alpha_r }{r!}\sum\limits_{q=0}^{l-2}\lambda^{qm}\e^{-\lambda M (q+1)}\sum\limits_{t=0}^s\binom{s}{t}K^{-t}t!\Big\{\lambda^m\frac{((q+1)M-K)^{(q+1)m-r+t}}{((q+1)m-r+t)!}- \lambda^r\frac{((q+1)M-K)^{qm+t}}{(qm+t)!}\Big\}
\label{eq:alpha_last2terms}
\end{equation}
Next, we get $I_1(s)$ defined at the beginning of this appendix as $I_1(s)=\int_{u=0}^{M}(K-u)^s\e^{\lambda u}g(u)\dd u$, where in the range $0<u<M$, $g(u)=g_{l-1}(u)$ given in (\ref{eq:g1_OO}). Substituting $g_{l-1}(u)$ in $I_1(s)$, we get
\begin{equation}
\begin{aligned}
I_1(s)=&\sum\limits_{r=0}^{m-1}\frac{\alpha_r}{r!}\Biggg[\sum\limits_{q=0}^{l-2}\lambda^{(q+2)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{(q+1)m-r-1}\frac{((q+1)M-K)^{(q+1)m-r-1-t}}{((q+1)m-r-1-t)!(m+t)!}F'(t,s)\\
&-\lambda^r\sum\limits_{q=1}^{l-2}\lambda^{(q+1)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{qm-1}\frac{((q+1)M-K)^{qm-1-t}}{(qm-1-t)!(m+t)!}F'(t,s)\Biggg]\end{aligned}
\label{eq:I_1_s_step1}
\end{equation}
where 
\begin{equation}
F'(t,s)=\int\limits_{u=0}^{M}(K-u)^s C(u,t)\dd u=\sum\limits_{b=0}^{s}\binom{s}{b}(K-M)^{s-b}\underbrace{\int\limits_{u=0}^M(M-u)^b C(u,t)\dd u}_{I_C(t,b)}.
\label{eq:F_dash_t_s}
\end{equation}
To solve $I_C(t,b)$, we first expand the gamma function in (\ref{eq:C_x_t}) and replace $\e^{\lambda\e^{\J\eta_k} u}\gamma\Big(m+t+1,\lambda\e^{\J\eta_k}u\Big)$ by $(m+t)!\Big[\e^{\lambda\e^{\J\eta_k}u}-\sum\limits_{w=0}^{m+t}\frac{\Big(\lambda\e^{\J\eta_k} u\Big)^w}{w!}\Big]$. We then solve integrals of the form $\int_{u=0}^M(M-u)^b u^n \dd u=\frac{M^{n+b+1}b!n!}{(n+b+1)!}$ once at $n=m+t$ and once at $n=w$, and an integral of the form $\int_{u=0}^{M}(M-u)^b\e^{\beta u}\dd u=\e^{M\beta}\beta^{-b-1}\gamma(b+1,M\beta)$ at $\beta=\lambda\e^{\J\eta_k}$. Substituting back in (\ref{eq:F_dash_t_s}), $F'(t,s)/(m+t)!$ reduces to $F(t,s)$ in (\ref{eq:F_t_s}).

Combining (\ref{eq:alpha_last2terms}) and $I_1(s)$ in (\ref{eq:I_1_s_step1}), $\alpha_s$ in (\ref{eq:alpha_r_definition}) reduces to 
\begin{equation}
\alpha_s=I_1(s)+I_2(s)+M^s\e^{-\lambda M}\sum\limits_{r=0}^{m-1}\alpha_r\frac{\lambda^r}{r!} \definedas \sum\limits_{r=0}^{m-1}\alpha_r d_{sr}, \quad s=0,\ldots,m-1,
\label{eq:alpha_s_dsr2}
\end{equation}
where $d_{sr}$ is given by
\begin{equation}
\begin{aligned}
d_{sr}&=-\frac{K^s }{r!}\sum\limits_{q=0}^{l-2}\lambda^{qm}\e^{-\lambda M (q+1)}\sum\limits_{t=0}^s\binom{s}{t}K^{-t}t!\Big\{\lambda^m\frac{((q+1)M-K)^{(q+1)m-r+t}}{((q+1)m-r+t)!}- \lambda^r\frac{((q+1)M-K)^{qm+t}}{(qm+t)!}\Big\}\\
&+\frac{1}{r!}\Biggg[\sum\limits_{q=0}^{l-2}\lambda^{(q+2)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{(q+1)m-r-1}\frac{((q+1)M-K)^{(q+1)m-r-1-t}}{((q+1)m-r-1-t)!}F(t,s)\\
&-\lambda^r\sum\limits_{q=1}^{l-2}\lambda^{(q+1)m}\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{qm-1}\frac{((q+1)M-K)^{qm-1-t}}{(qm-1-t)!}F(t,s)\Biggg]
\end{aligned}
\label{eq:dsr_appendix}
\end{equation}
Equation (\ref{eq:alpha_s_dsr2}) forms a homogeneous system of linear equations in $\alpha$ which has infinite number of solutions. In order to obtain the unique solution for $\alpha_r$, $r=0,\ldots,m-1$, and therefore the unique energy distribution, we additionally use the unit area equation $\int_{u=0}^K g(u)\dd u + \pi(K)=1$, which can be written as
\begin{equation}
\underbrace{\int\limits_{u=0}^M g_{l-1}(u)\dd u}_{I_{\text{U1}}} +\underbrace{\int\limits_{u=M}^K g(u)\dd u + \pi(K)}_{I_{\text{U2}}}\definedas \sum\limits_{r=0}^{m-1}\alpha_r a_{r}=1
\label{eq:unit_area_OO}
\end{equation}
$I_{\text{U2}}$ can be obtained in a similar manner used to get (\ref{eq:area_under_g_step4}). Specifically, since the pdf $g(x)$ for the on-off scheme in the range $M<x<K$ in (\ref{eq:g2_OO}) is identical to the pdf of the best-effort scheme in (\ref{eq:pdf_Nakagami_m}). The integral $\int_{u=M}^K g(u)\dd u$ is identical to the right hand side (R.H.S) of (\ref{eq:area_under_g}) with the last term replaced by $\int_{u=M}^{K-(l-2)M}g_{l-2}(u)\dd u$. Consequently,  $\int_{u=M}^K g(u)\dd u$ is same as the R.H.S. of (\ref{eq:area_under_g_step2}) after replacing the upper limit of the inner summations by $q=l-2$ and the inner lower integral limit by $M$. Thus, the inner integrals have the form $\int_{u=M}^{b}\e^{-\lambda u}\Big(u-b\Big)^c/c!\dd u=-\lambda^{-c-1}\Big[\e^{-\lambda b}-\e^{-\lambda M}\sum_{t=0}^{c}(\lambda(M-b))^t/t!\Big]$, at $b=K-qM$ and at $c=(q+1)m-r-1$ in the first term and $c=qm-1$ in the second term. These considerations lead to 
\begin{equation}
\begin{aligned}
\int\limits_{u=M}^K g(u)\dd u&=\sum\limits_{r=0}^{m-1}\frac{\alpha_r}{r!}\Biggg[\sum\limits_{q=0}^{l-2} -\lambda^r\Biggg(\e^{-\lambda K}-\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{(q+1)m-r-1}\frac{\Big(\lambda((q+1)M-K)\Big)^t}{t!}\Biggg)\\
 &+\sum\limits_{q=1}^{l-2} \lambda^r\Biggg(\e^{-\lambda K}-\e^{-\lambda M(q+1)}\sum\limits_{t=0}^{qm-1}\frac{\Big(\lambda((q+1)M-K)\Big)^t}{t!}\Biggg)\Biggg]
\end{aligned}
\label{eq:area_g_K_M}
\end{equation}
Separating $q=0$ in the first term in (\ref{eq:area_g_K_M}), $\int\limits_{u=M}^K g(u)\dd u$ reduces to \small
\begin{equation}
\sum\limits_{r=0}^{m-1}\frac{\alpha_r}{r!}\Biggg[ \lambda^r\Biggg(-\e^{-\lambda
 K}+\e^{-\lambda M}\sum\limits_{t=0}^{m-r-1}\frac{\Big(\lambda(M-K)\Big)^t}{t!}\Biggg)
 +\sum\limits_{q=1}^{l-2} \lambda^r\e^{-\lambda
 M(q+1)}\sum\limits_{t=qm}^{(q+1)m-r-1}\frac{\Big(\lambda((q+1)M-K)\Big)^t}{t!}\Biggg]
\label{eq:area_g_K_M2}
\end{equation}
\normalsize
From (\ref{eq:Pi_K_Nakagami_OO}), the first term in (\ref{eq:area_g_K_M2}) is $-\pi(K)$. The second term in (\ref{eq:area_g_K_M2}) is equivalent to the summand in the third term at $q=0$. Hence, we can write
\begin{equation}
I_{\text{U2}}=\int\limits_{u=M}^K g(u)\dd u + \pi(K)=\sum\limits_{r=0}^{m-1}\frac{\alpha_r \lambda^r}{r!}\sum\limits_{q=0}^{l-2}\e^{-\lambda M(q+1)}\sum\limits_{t=qm}^{(q+1)m-r-1}\frac{\lambda^t((q+1)M-K)^{t}}{t!}
\label{eq:area_g_K_M3}
\end{equation}
Having obtained $I_{\text{U2}}$, it remains to obtain $I_{\text{U1}}=\int_{u=0}^M g_{l-1}(u)\dd u$. Using $g_{l-1}(u)$ in (\ref{eq:g1_OO}), $I_{\text{U1}}$ is identical to $I_1(s)$ in (\ref{eq:I_1_s_step1}) with $F'(t,s)$ replaced by $H'(t)$ given by $H'(t)=\int_{u=0}^{M}e^{-\lambda u} C(u,t)\dd u$. Similar to the analysis of $I_C(t,b)$ in (\ref{eq:F_dash_t_s}), we first expand the gamma function in (\ref{eq:C_x_t}) and replace $\e^{\lambda\e^{\J\eta_k} u}\gamma\Big(m+t+1,\lambda\e^{\J\eta_k}u\Big)$ by $(m+t)!\Big[\e^{\lambda\e^{\J\eta_k}u}-\sum_{w=0}^{m+t}\frac{\Big(\lambda\e^{\J\eta_k} u\Big)^w}{w!}\Big]$. We then solve integrals of the form $\int_{u=0}^{M}\e^{-\lambda u} u^n=\lambda^{-n-1}\gamma(n+1,\lambda M)$ once at $n=m+t$ and once at $n=w$, and an integral of the form $\int_{u=0}^M \e^{-\lambda u (1-\e^{\J\eta_k})}\dd u$ which results in $M$ at $k=0$ and $\Big(1-\e^{-\lambda M (1-\e^{\J\eta_k})}\Big) \Big(\lambda(1-\e^{\J\eta_k})\Big)^{-1}$, otherwise. With these considerations, $H(t)=H'(t)/(m+t)!$ reduces to (\ref{eq:H_T}). Having obtained $I_{\text{U1}}$ and $I_{\text{U2}}$, $a_r$ in (\ref{eq:unit_area_OO}) can be concluded. Adding (\ref{eq:unit_area_OO}) to (\ref{eq:alpha_s_dsr2}), we get $\alpha_s+\sum\limits_{r=0}^{m-1}\alpha_r(a_r-d_{sr})=1$ which forms a non-homogeneous system of linear equations whose solution is given after (\ref{eq:Pi_K_Nakagami_OO}). This completes the proof. 


==> Infinite_buffer.tex <==
Studying an infinite-size energy buffer is of interest since the harvested energy can be several orders of magnitude lower than the capacity of commonly-used energy buffers, e.g. rechargeable batteries. In this section, we consider an infinite-size energy buffer and study the energy storage processes in (\ref{eq:general_storage_equation_BE}) and (\ref{eq:general_storage_equation_OO}) corresponding to the best-effort and the on-off transmission policies, respectively.  We provide conditions under which the convergence of the amount of stored energy to a limiting distribution is either guaranteed or violated. Furthermore, for both storages processes  (\ref{eq:general_storage_equation_BE}) and (\ref{eq:general_storage_equation_OO}), we derive the general integral equations for the  limiting distribution of the stored energy and provide their solution in closed form for a Nakagami-$m$ block fading DL channel.\vspace{-0.5cm}% and when the EH process is i.i.d. exponentially distributed,  i.e., for a Rayleigh block fading DL channel.%, i.e., $K\to\infty$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Existence of a Limiting Energy Distribution}
\begin{theorem}\normalfont
For the storage processes $\{B(i)\}$ in (\ref{eq:general_storage_equation_BE}) and (\ref{eq:general_storage_equation_OO}) with an infinite-size energy buffer, if the maximum output energy of the buffer is less than the average harvested input energy to the buffer, i.e., if $M<\bar{X}$, then $\{B(i)\}$ does not possess a stationary distribution. Furthermore, after a finite number of time slots, $\Pul(i)=M$ holds almost surely (a.s.).
\label{theo:no_stationary_dist}
\end{theorem}\vspace{-0.4cm}
\ifARXIV
\begin{proof} The proof is provided in Appendix \ref{app:no_stationary_dist} and in \cite[Appendix A]{Morsi_ICC2015}. \end{proof}
\else
\begin{proof} The proof is provided in \cite[Appendix A]{Morsi_storage_arxiv} and  \cite[Appendix A]{Morsi_ICC2015}. %It applies for both the best-effort and the on-off policies. 
\end{proof}
\fi\vspace{-0.3cm}
%\begin{lemma}\normalfont
%For the storage process $\{B(i)\}$ in (\ref{eq:general_storage_equation}) with infinite buffer size, if $\{B(i)\}$ possesses a stationary distribution, then $\E[\Pul(i)]=\bar{X}$.
%\label{lemma:avg_Pul_Xbar}
%\end{lemma}
%\begin{proof} The proof is provided in Appendix \ref{app:avg_Pul_Xbar} \end{proof}
\begin{theorem}\normalfont
For the storage processes $\{B(i)\}$ in (\ref{eq:general_storage_equation_BE}) and (\ref{eq:general_storage_equation_OO}) with an infinite-size energy buffer, if the maximum output energy of the buffer is larger than the average harvested input energy to the buffer, i.e., if $M>\bar{X}$, then $\{B(i)\}$ is a stationary and ergodic process which possesses a unique stationary distribution $\pi$ that is absolutely continuous on $(0,\infty)$. Furthermore, the process converges in total variation to the limiting distribution $\pi$ from any initial distribution. In addition, $\E[\Pul(i)]=\bar{X}$ holds.
\label{theo:stationary_dist_infinite}
\end{theorem}\vspace{-1.1cm}
\ifARXIV
\begin{proof} The proof is provided in Appendix \ref{app:stationary_dist_infinite_BE} and  partially in \cite[Appendix B]{Morsi_ICC2015}.% and \ref{app:stationary_dist_infinite_OO} for the best-effort and the on-off policies, respectively. 
\end{proof}
\else
\begin{proof} The proof is provided in \cite[Appendix B]{Morsi_storage_arxiv} and partially in \cite[Appendix B]{Morsi_ICC2015}. \end{proof}
\fi \vspace{-0.7cm}%\cite[Appendix B]{Morsi_ICC2015} and
%From Remark \ref{remark:equivalence_to_Morans_Model}, it can be observed that Moran's process $\{Z(i)\}$ in (\ref{eq:Moran_buffer_content}) is equivalent to the waiting time of a customer in a GI/G/1 queue \cite{asmussen2003applied}, where $X(i)$ is equivalent to the customer service time and $M$ is equivalent to the customers' inter-arrival time. Now, our storage process $\{B(i)\}$ in (\ref{eq:general_storage_equation_BE}) with $K\!\to\!\infty$ is equivalent to the process $U(i)=Z(i)+X(i)$, see (\ref{eq:U_i_process}). That is, $\{B(i)\}$ is equivalent to the sojourn time (waiting time plus service time) of a customer in a GI/G/1 queue. Since $\{Z(i)\}$ and $\{X(i)\}$ are independent and $\{X(i)\}$ is stationary, then the steady state behavior of $\{B(i)\}$ is solely governed by that of $\{Z(i)\}$. Hence, from \cite[Corollary 6.5 and Corollary 6.6]{asmussen2003applied}, $M>\bar{X}$ is a sufficient condition for the process $\{Z(i)\}$ and thus for $\{B(i)\}$ to possess a unique stationary distribution to which it converges in total variation from any initial distribution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Best-Effort Policy with an Infinite-Size Energy Buffer}
\label{ss:BE_scheme_INF}
\begin{theorem}\normalfont
Consider the storage process $\{B(i)\}$ of the best-effort policy in (\ref{eq:general_storage_equation_BE}) with an infinite-size energy buffer and $M>\bar{X}$. Let $g(x)$ on $(0,\infty)$ be the limiting pdf of the stored energy. If $f(x)$ and $F(x)$ are respectively the pdf and the cdf of the EH process $\{X(i)\}$, then $g(x)$ must satisfy the following integral equation\vspace{-0.3cm}
\begin{equation}
g(x)=f(x)\int\limits_0^M g(u) \dd u + \int\limits_M^{M+x} f(x-u+M) g(u) \dd u,
\label{eq:Integral_eqn_infinite_BE}
\end{equation}
and the limiting cdf $G(x)$ of the stored energy satisfies the following Lindley integral equation
\begin{equation}
G(x)=\int\limits_{u=0}^x G(x-u+M)\dd F(u).
\label{eq:CDF_Integral_eqn_infinite_BE}
\end{equation}
\label{theo:integral_eq_infinite_BE}
\end{theorem}
%%%%%
\vspace{-0.9cm}
\begin{proof}
\ifARXIV
The proof is provided in Appendix \ref{app:proof_BE_integral_eqn_infinite} and partially in \cite[Proof of Theorem 3]{Morsi_ICC2015}.
\else
The proof is provided in \cite[Appendix C]{Morsi_storage_arxiv} and partially in \cite[Proof of Theorem 3]{Morsi_ICC2015}.
\fi
\end{proof} \vspace{-0.2cm}
%%%%%%%%%%
Next, we consider the case when the DL channel is Nakagami-$m$ block fading, i.e., the EH process is Gamma distributed\footnote{We note that when the harvested power is Gamma distributed with shape parameter $m$, then the DL channel power gain $\hdl(i)=X(i)/\eta\Pdl$ is also gamma distributed with the same shape parameter $m$.\vspace{-0.6cm}}.%In the following corollary, we provide the limiting distribution of the stored energy. \vspace{-0.3cm}
 \vspace{-0.3cm}\begin{corollary}\normalfont %[Energy Distribution in Infinite-size buffer using best-effort policy] 
Consider the storage process $\{B(i)\}$ of the best-effort policy in (\ref{eq:general_storage_equation_BE}) with an infinite-size energy buffer and $M\!>\!\bar{X}$. If the EH process $\{X(i)\}$ is Gamma distributed with an integer shape parameter $m\in\{1,2,\ldots\}$ and pdf $f(x)\!=\!\frac{\lambda^m}{\Gamma(m)}x^{m-1}\e^{-\lambda x}$, where $\lambda\!\!=\!\!m/\bar{X}$  and $\delta\!=\!M/\bar{X}=\lambda M/m$, then the stored energy has a limiting cdf given by $G(x)\!\!=\!\!1-\sum_{n=0}^{m-1}c_n\e^{-\lambda_n x}$ and a limiting pdf given by $g(x)\!\!=\!\!\sum_{n=0}^{m-1}\lambda_n c_n\e^{-\lambda_n x}$, where $\lambda_n\!=\lambda+\frac{m}{M} W_0\left(-\delta \e^{-\delta}\e^{-\J\frac{2 \pi n}{m}}\right)$. The coefficients $c_n$, $n=0,\ldots,m-1$, are obtained by solving the non-homogeneous system of linear equations $\V{A} \V{c}=\V{1}_m$, where $\V{c}=[c_0,\ldots,c_{m-1}]^T$ and $\V{A}$ is an $m\times m$ matrix whose entry in the $s^{\text{th}}$ row and the $n^{\text{th}}$ column is given by $A_{s,n}=\left(\frac{\lambda-\lambda_n}{\lambda}\right)^s$, where $s,n\in\{0,\ldots,m-1\}$.
\label{theo:stationary_dist_infinite_Nakagami}
\end{corollary} \vspace{-0.4cm}
% For both IEEE and ARXIV Versions
\begin{proof} The proof is provided in Appendix \ref{app:stationary_dist_infinite_Nakagami_BE}. \end{proof} \vspace{-0.3cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\subsection{On-Off Policy with an Infinite-Size Energy Buffer}
\label{ss:OO_scheme_INF}
\begin{theorem}\normalfont
Consider the storage process $\{B(i)\}$ of the on-off policy in (\ref{eq:general_storage_equation_OO}) with an infinite-size energy buffer and $M>\bar{X}$. Let $g(x)$ on $(0,\infty)$ be the limiting pdf of the stored energy. If $f(x)$ is the pdf of the EH process $\{X(i)\}$, then $g(x)$ must satisfy the following integral equation\vspace{-0.1cm}
\begin{numcases}{g(x)\!=\!\! \label{eq:g_integral_eqn_infinite_OO}}
\int\limits_{u=0}^x f(x-u) g(u) \dd u + \int\limits_{u=M}^{M+x} f(x-u+M) g(u) \dd u, &  $0\leq x< M$ \label{eq:Integral_eqn_infinite_parta_OO}\\
\int\limits_{u=0}^M f(x-u)g(u) \dd u + \int\limits_{u=M}^{M+x} f(x-u+M) g(u) \dd u,  &  $x\geq M$  \label{eq:Integral_eqn_infinite_partb_OO}\end{numcases}
\label{theo:OO_integral_eqn_infinite}
\end{theorem}\vspace{-0.8cm}
\ifARXIV
\begin{proof} The proof is provided in Appendix \ref{app:proof_OO_integral_eqn_infinite} and in \cite[Proof of Theorem 3]{Morsi_Asilomar2014}. \end{proof}
\else
\begin{proof} The proof is provided in \cite[Appendix E]{Morsi_storage_arxiv} and \cite[Proof of Theorem 3]{Morsi_Asilomar2014}. \end{proof}
\fi
%To understand the integral equation in (\ref{eq:g_integral_eqn_infinite_OO}), one may set $B(i)=u$ and $B(i+1)=x$, then (\ref{eq:general_storage_equation_OO}) with $K\to\infty$ reads \small $x=\begin{cases} u+X(i), & u\leq M \\ u-M+X(i), & u>M \end{cases}.$ \normalsize
%%\vspace{-0.1cm}
%%\begin{equation}
%%x=\begin{cases} u+X(i), & u\leq M \\ u-M+X(i), & u>M \end{cases}.\vspace{-0.1cm}
%%\label{eq:Storage_eq_Infinite_u_x_OO}
%%\end{equation}
%Thus, for $u\leq M$, $g(x|u\leq M)=f(x-u)$ which is non-zero only for a non-negative amount of harvested energy, i.e., for $u\leq x$. Hence, in the range $u\leq M$, the upper limit on $u$ in the first integral of (\ref{eq:Integral_eqn_infinite_parta_OO}) and (\ref{eq:Integral_eqn_infinite_partb_OO}) is given by $u=\min(x,M)$. The second integral in (\ref{eq:Integral_eqn_infinite_parta_OO}) and (\ref{eq:Integral_eqn_infinite_partb_OO}) corresponds to the range $u>M$. In this case, $g(x|u> M)=f(x-u+M)$ which is non-zero only for a non-negative amount of harvested energy, i.e., for $u\leq M+x$. This completes the proof. %These considerations lead to (\ref{eq:Integral_eqn_infinite}).% \vspace{-0.3cm}%This explains the upper limit in the integral of the second term of (\ref{eq:Integral_eqn_infinite}).  and 
%\end{proof\vspace{-0.2cm}
%%%%%%%%%%
Next, we consider the case when the DL channel is Nakagami-$m$ block fading, i.e., the EH process is Gamma distributed.% and provide the limiting distribution of the stored energy in the following corollary.
%%%%%%%%%%%%%%%%% ON-OFF Infinite Nakagami
\begin{corollary} \normalfont
Consider the storage process $\{B(i)\}$ of the on-off policy in (\ref{eq:general_storage_equation_OO}) with an infinite-size energy buffer and $M\!>\!\bar{X}$. If the EH process $\{X(i)\}$ is Gamma distributed with an integer shape parameter $m\in\{1,2,\ldots\}$ and pdf $f(x)\!=\!\frac{\lambda^m}{\Gamma(m)}x^{m-1}\e^{-\lambda x}$, where $\lambda\!\!=\!\!m/\bar{X}$  and $\delta\!=\!M/\bar{X}=\lambda M/m$, then the stored energy has a limiting pdf given by
%\begin{equation}
%\begin{aligned}
%\sum\limits_{n=0}^{m-1} -\lambda_n c_n\Biggg[\e^{-\lambda_n x}+\frac{\lambda}{m}\sum\limits_{k=0}^{m-1}\frac{1}{b_{nk}} \Bigg\{ & \e^{-\lambda x[1-\cos(\eta_k)]}\Big((\lambda_n-\lambda)\cos(\eta_k+\lambda x \sin(\eta_k))+\\
%& \lambda\cos(\lambda x \sin(\eta_k))\Big)+a_{nk}\e^{-\lambda_n x}\Bigg\} \Biggg],
%\end{aligned}
%\end{equation}
\begin{numcases}{\hspace{-1.5cm}g(x)\!=\!\! \label{eq:PDF_INF_BE_Nakagami}}
\begin{aligned}
\!\!\!&\sum\limits_{n=0}^{m-1} \lambda_n c_n\Biggg[ \e^{-\lambda_n x}+\frac{\lambda}{m}\sum\limits_{k=0}^{m-1}\frac{1}{b_{nk}}  \Bigg\{\e^{-\lambda x[1-\cos(\eta_k)]}\\[-2.5ex]
&\Big((\lambda_n-\lambda)\cos(\eta_k+\lambda x \sin(\eta_k))+\lambda\cos(\lambda x \sin(\eta_k))\Big)+a_{nk}\e^{-\lambda_n x}\Bigg\}\\[-2.5ex]
&\!\!\!-\!\sum\limits_{t=0}^{m-1}\frac{(\lambda\!-\!\lambda_n)^t}{t!}\e^{-\lambda x}\Bigg\{x^t\!+\! \frac{1}{m}\sum\limits_{k=0}^{m-1}\Re\{(\lambda\e^{\J\eta_k})^{-t}\e^{\lambda x\e^{\J\eta_k}}\gamma(t\!+\!1,\lambda x\e^{\J\eta_k})\}\Bigg\}\Biggg],
\end{aligned} & \hspace{-0.5cm}$0\!\leq \!x\!<\!\!M$ \label{eq:g1_INF_OO}\\
\sum\limits_{n=0}^{m-1} \lambda_n c_n\e^{-\lambda_n x},  &  \hspace{0cm}$x\!\geq\! M$  \label{eq:g2_INF_OO}\end{numcases}
where $\eta_k=\frac{2\pi k}{m}$, $a_{nk}=(\lambda-\lambda_n)\cos(\eta_k)-\lambda$, $b_{nk}=2\lambda(\lambda-\lambda_n)(1-\cos(\eta_k))+\lambda_n^2$, and $\lambda_n\!=\lambda+\frac{m}{M} W_0\left(-\delta \e^{-\delta}\e^{-\J\frac{2 \pi n}{m}}\right)$.  The coefficients $c_n$, $n=0,\ldots,m-1$, are obtained by solving the system of linear equations $\V{A} \V{c}=\V{1}_m$, where $\V{c}=[c_0,\ldots,c_{m-1}]^T$ and $\V{A}$ is an $m\times m$ matrix whose entry in the $s^{\text{th}}$ row and the $n^{\text{th}}$ column, for $s,n\in\{0,\ldots,m-1\}$, is given by $A_{s,n}=D_n+B_{sn}$, where
\begin{equation}
\begin{aligned}
D_n&=\frac{\lambda_n\lambda}{m}\sum\limits_{k=0}^{m-1}\frac{1}{b_{nk}}\Big(\beta_{nk}+\frac{a_{nk}}{\lambda_n}(1-\e^{-\lambda_n M})\Big)
-\lambda_n\sum\limits_{t=0}^{m-1}(\lambda-\lambda_n)^t\Biggg\{\frac{\lambda^{-t-1}}{t!}\gamma(t+1,\lambda M)\\[-1ex]
&+\frac{1}{m}\sum\limits_{k=0}^{m-1}\Re\Bigg\{(\lambda\e^{\J\eta_k})^{-t}\Bigg[\zeta_k
-\sum\limits_{q=0}^{t}\frac{\e^{\J\eta_k q}\lambda^{-1}}{q!}\gamma(q+1,\lambda M)\Bigg]\Bigg\}\Biggg\}+1,
\end{aligned}
\label{eq:D_n_OO}
\end{equation}
with \vspace{-0.2cm}
%\begin{aligned}
%&\frac{1}{2\lambda^2[1-\cos(\eta_k)]}\Biggg(\e^{-\lambda M(1-\cos(\eta_k))}\Bigg\{\Big(\lambda_n\lambda -2\lambda^2\Big)\Big(1-\cos(\eta_k)\Big)\cos(\lambda M\sin(\eta_k))\\
%&+\lambda_n\lambda\sin(\eta_k)\sin\Big(\lambda M \sin(\eta_k)\Big)\Bigg\}+(2\lambda^2-\lambda_n\lambda)(1-\cos(\eta_k))\Biggg)
\begin{equation*}
\beta_{nk}=
\begin{cases}
\lambda_n M & k\!=\!0\\
\e^{-\lambda M(1-\cos(\eta_k))}\Bigg[\frac{\lambda_n\lambda\Big(\cos\left(\lambda M \sin(\eta_k)\right)-\cos(\eta_k+\lambda M \sin(\eta_k))\Big)}{2\lambda^2[1-\cos(\eta_k)]}\! -\!\cos\left(\lambda M \sin(\eta_k)\right)\Bigg]\!+\!1\!-\!\frac{\lambda_n}{2\lambda}
 &k\!\neq\! 0
\end{cases}
\end{equation*}\vspace{-0.2cm}
and $\zeta_{k}=
\begin{cases}
M & k=0\\
\frac{1-\e^{-\lambda M(1-\e^{\J\eta_k})}}{\lambda(1-\e^{\J\eta_k})}
 &k\neq 0
\end{cases}
$,
\begin{equation}
\begin{aligned}
&B_{sn}=-\lambda_n(\lambda-\lambda_n)^s+\frac{\lambda^m(-1)^{m-1-s}\lambda_n}{(m-1-s)!}\Biggg[\left( 1+\frac{\lambda}{m}\sum\limits_{k=0}^{m-1} \frac{a_{nk}}{b_{nk}}\right)(\lambda_n-\lambda)^{-m+s}\gamma\big(m-s,(\lambda_n-\lambda)M\big)\\
&+\frac{\lambda}{m}\sum\limits_{k=0}^{m-1}\Biggg(\frac{1}{b_{nk}}\big((\lambda_n-\lambda)\cos(\eta_k)+\lambda\big)\Re\{I_{\text{complex}}\}
+\frac{1}{b_{nk}}\big((\lambda_n-\lambda)\sin(\eta_k)\big)\Im\{I_{\text{complex}}\}\Biggg)\\
&-\sum\limits_{t=0}^{m-1}\frac{(\lambda-\lambda_n)^{t}}{t!}\Bigg\{\frac{M^{m+t-s}}{(m+t-s)}+\frac{1}{m}\sum\limits_{k=0}^{m-1}\Re\Big\{(\lambda\e^{\J\eta_k})^{-t}t!\Big[I_{\text{complex}}^*
-\sum\limits_{q=0}^{t}\frac{(\lambda\e^{\J\eta_k})^q}{q!}\frac{M^{m+q-s}}{(m+q-s)}\Big]\Big\}\Bigg\}\Biggg],
\end{aligned}
\label{eq:B_sn_OO}
\end{equation}
with $I_{\text{complex}}=(-\lambda\e^{-\J\eta_k})^{-m+s}\gamma\big(m-s,-\lambda M\e^{-\J\eta_k}\big)$.
\label{theo:stationary_dist_infinite_Nakagami_OO}
\end{corollary} \vspace{-0.3cm}
\ifARXIV
\begin{proof} The proof is provided in Appendix \ref{app:stationary_dist_infinite_Nakagami_OO}. \end{proof}
\else
\begin{proof} The proof is provided in Appendix \ref{app:stationary_dist_infinite_Nakagami_OO_shortened} and is given in more detail in \cite[Appendix F]{Morsi_storage_arxiv}. \end{proof}\vspace{-0.3cm}
\fi
%%%%%%%%%%%%
\begin{remark} \normalfont
The limiting distribution of the energy stored in an infinite-size energy buffer for the best-effort and the on-off policies obtained in Corollaries \ref{theo:stationary_dist_infinite_Nakagami} and \ref{theo:stationary_dist_infinite_Nakagami_OO} are real-valued despite the complex-valued parameters $\lambda_n$ and $c_n$. Furthermore, $\lambda_{n}\!=\!\lambda_{m-n}^*$ and $c_{n}\!=\!c_{m-n}^*$, $\forall$ $n\!=\!1,\ldots,\frac{m}{2}\!-\!1$  if $n$ is even and $\forall$ $n\!=\!1,\ldots,\frac{m-1}{2}$, if $n$ is odd.
\label{coro:real_valued_pdfs}
\end{remark}\vspace{-0.2cm}
\ifARXIV
\begin{proof} The proof is provided in Appendix \ref{app:real_valued_pdfs}. \end{proof}
\else
\begin{proof}
The proof is provided in \cite[Appendix G]{Morsi_storage_arxiv}.
\end{proof}\vspace{-0.4cm}
\fi
%Next, we consider the case when the DL channel is Rayleigh block fading and provide the limiting distribution of the stored energy in the following corollary.
%\begin{remark} \normalfont
%In the special case of a Rayleigh fading DL channel, the EH process is exponentially distributed, i.e., $m=1$ in Corollary \ref{theo:stationary_dist_infinite_Nakagami} with pdf $f(x)\!=\!\lambda \e^{-\lambda x}$, where $\lambda\!\!=\!\!\frac{1}{\bar{X}}$  and $\delta\!=\!\lambda M\!=\!\frac{M}{\bar{X}}$, then the limiting pdf of the stored energy is $g(x)\!\!=\!\!p\e^{-p x}$, where $p\!>\!0$ is given by $p\!=\frac{\delta+W_{0}(-\delta\e^{-\delta})}{M}$ and $W_0(\cdot)$ is the principle branch of the Lambert W function. 
%\label{theo:stationary_dist_infinite_exp}
%\end{remark} %\vspace{-0.cm}
%\begin{proof} The proof is provided in Appendix \ref{app:stationary_dist_infinite_exp}. \end{proof}


==> To_include_in_revision.tex <==
 1- Emphasize that to the best of our knowledge we are the first to use a continuous-state Markov chain in modeling the stored energy in an energy harvesting communication system.
 2- Also emphasize that we show that buffering energy improves the system performance significantly compared to using the harvested energy on a slot by slot basis.
 3- Emphasize clearly that our analysis is not only valid for energy harvested through wireless power transfer, but is valid also for energy harvested from any renewable energy source if the amount of harvested energy is i.i.d. gamma distributed. This also holds especially that we assume that energy is havresting and information is tranmsmitted simultaneously, which is the case with conventional opportunistic energy harvesting models. If with wireless power transfer, we assume that the time slot is dividd mong energy harvesting and information transmission, then this won't make sense in the case when the harvested energy is from solar power, since harvesting energy from the solar cell does not interfere with transmitting energy from the sensor node.
 
 Q: can solar energy be studied in a slotted manner, with the harvested energy among the slots be i.i.d. or must it be studied with the intermittent (sporadic) energy arrival nature, assuming either deterministic arrivals or Poisson distributed stochastic arrivals.
 
 3- I probably need to refer to "Implications of Energy Profile and Storage on
Energy Harvesting Sensor Link Performance" which also uses a markov model for EH and analyzes the outage probability as a function of the nodes transmit power showing very similar curves
4- If possible, mention that we only consider energy consumption in communication, whereas energy consumption due to sensing is not considered. 

==> To_include_oct_2016.tex <==
recent papers including wireless power transfer with energy storage

?? closed-form expressions for outage probability with the BE scheme? (just final resul\t)

ddiversity order....refer to paper by gianikis as it is the only one talking about diversity orders in siso systems and studying them at high SNR

For the given simulation parameters, plot BE pdf and On-Off pdf for m=2 and atoms for infinite and finite cases

In BE finite case, check if the equations are also valid for K=lM


Replace cn by-cn to get nigher looking pdf eqn and also cdf equation, cdf=1-... and pdf=sum of positive looking terms.
Update the equations accordingly

In our model, we assume that the AP transmits energy and receives information form the EH node simultaneously. This means it is a hybrid access point (hybrid because it receives information and transmits energy) operating at the full-duplex mode (because both transmission and reception are done simultaneously, so the HAP needs 2 antennas for this). However, in our case, we also assume that the EH node harvests energy and transmits information simultaneously. This means that also the EH node needs 2 antennas :(, this might be however not practical for a simple sensor node. We additionally assume that the EH node uses the harvested energy only in future time slots.

Include the main condtributions of the paper and motivate for how different and nicer is this work compared to previous work. It seems for example that no one considered continuous state markov chains before.

Include this paper "A Discrete Time-Switching Protocol for Wireless-Powered Communications with Energy Accumulation" 
How different it is from our work
1- it assumes that the AP has multiple antennas...not an issue
2- It assumes that the EH node doesn't harvest energy and transmits information simultaneously. This is a practical assumption as EH nodes are usually simple with only one antenna. OOhh and for self-interference avoidance, we should assume that energy transfer and information transfer use different frequency bands. 
3- The paper assumes that the EH node knows the UL channel, so it accumulates energy until its energy is sufficient for an outage free transmission, which the node can assess since it knows the UL channel. In our case for practical reasons, we assume that the node has no knowledge of the UL CSI, so with the on-off protocol the node accumulates energy just until it reaches energy level M, and M is a design parameter which can be optimized for given the buffer size and the average channel conditions. 
4- This paper uses discrete Markov chains to study the energy storage behaviour.
5- This paper provide outage probability results but for Rayleigh fading
So in the introduction we need to state explicitly that unlike most previous works, we assume continuous-state Markov chains.



We really need to compare our results with one or more previous work in which our work is superior. This needs time but if our policy  performs for example (even if worse) but close to another optimal policy that needs channel knowledge, this will make our paper stronger for citations. 

--Also emphasize the we assume Nakagami-m fading channels which is a general channel model that can be used to describe Ricean fading, Rayleigh fading as well as other practical channel models.  We should also emphasize that our analysis is not just valid for WPT but also for any energy harvesting source in which the energy emitted is IID gamma distributed.

--Also emphasize that in our paper, we considers imperfections
--To define b(i), use the term residual amount of energy stored in the energy buffer

-- note that here we assume gamma distribution, that means m is integer, and from WIki if m is positive integer, then the distribution represents an Erlang distribution; i.e., the sum of k independent exponentially distributed random variables, each of which has a mean of θ.
-- Also state that using the gamma distribution assumption of the downlink channel, means that for a positive integer m, the Dl channel is Erlang distribution ie., sum of exponentially distributed RVs with mean 1/lambda. Hence, our model also describes the use of m-antenna AP that uses maximum ratio transmission (and thus has CSI knowledge of the DL channel) and transmits over m Rayleigh fading channels. This is for example the case considered in paper "A Discrete Time-Switching Protocol for Wireless-Powered Communications with Energy Accumulation"

-- In paper "A Discrete Time-Switching Protocol for Wireless-Powered Communications with Energy Accumulation" as well as another paper I reviewed as well as papers of imperfect CSI I worked on before, the authors use the term throughput to refer to the product of the constant rate R at which transmission occurs  times the probability of a non-outage event. We can use this metric instead of the outage

--In On-off scheme, explain that a large choice of M indicates that we will have more off slots, which increase the outage incidents and reduce the effective throughput, but at the same time it reduces the probability of outages in the on-slots. This indicates that there exists and optimal M at which the total outage and therefore the throughput is minimized.


---In the introduction. Discuss why buffering is useful compared to just using all the energy collected in a time slot for the information transmission in the subsequent time slot. From the outage probability perspective, when energy is buffered, then optimally the minimum power needed for outrage-free transmission can be used, while the remaining energy in the buffer can be stored to compensate for deep fades in future slots.

--In the simulations section Discuss that for both BE and OO schemes, an optimal M must exist. First for the BE scheme, if M is too small (relative to Xbar and K), it means that the maximum power the node transmits with (M) is small so more outage events occur. Now if we increase M way beyond Xbar, it means in many cases we harvest around X_bar so in many slots we just transmit with all the energy we harvested in the previous slot, so energy buffering is not actually of any use. In the extreme case, when M=K, we have a buffer-free EH node which in every time slot transmits with all the harvested energy in the previous time slot which does not make use of the energy buffer since in this case, we might transmit with a power much greater than that needed for an outage-free transmission, while transmitting with a non-sufficient power in future slots with deep fades. So buffering the excess energy for future slots is of course beneficial.
For the OO scheme, all the above holds + that smaller M means more on slots but also higher outage probability during on-slots, while larger M means more off slots (no-transmission outages) and less outage events during the on-slots. So here there is another dimension or reason for why there exists an optimal value for M

%%%%%%%%%%%Figures to include%%%%%%%%%%%
1- Throughput vs R at opt deltas
May be show this for 2 different pdl and for different m
Show the pdf of for the case of optimal M for the same parameters used to get the first figure for both on-off and BE
Show outage probability or throughput against SNR
compare with batteryless scheme


%%%% 
A note on although the equations look complicated, 1- the summations over l, K=lM, if l is too large one may use the simpler result of the infinite buffer. Also getting alpha r requires summations over m, which is in realistic systems small less than 4. also the matrix inversion needed is of size mxm which is small.
--In the simulations section, mention that beta scales the eta and alpga scales the gamma threshold and thus results in a more stringent requirement for outage-free transmission.
---We note that rounding l up or done has only effect of the summation limit but we use the exact K otherwise. Results are still close to exact. For a general K, the solution is tedious and not needed since rounding results in almost exact results.

Add a proof as to why the optimal delta at infinite buffer size is optimal for the outage probability.

--- Explain that the Best effort scheme tends to the batteryless scheme as M tends to infinity for an infinite size buffer.  You may also mention the this "outage floor" asymtotic result as Mtends to infinity. 

%%%%%%%%%%%%%%%
As a conclusion, we motivated that we want to study the best-effort and the on-off schemes to see which scheme behaves better and therefore expect an intermediate performance for the piece-wise constant scheme in between. Now, given that we got that the BE scheme is always better than the on-off scheme and less sensitive to the value of the maximum transmit power. The on-off scheme seems to only outperform the BE scheme at very high transmission rates (high outage threshold) which in general provide low throughput values. At the optimal transmission rate that maximizes the throughput, both schemes behave similarly. But the on-off scheme is very sensitive to changes in the transmit power. 

Can the optimal delta be more than 1 for the on-off and for the best effort scheme, and when does that happen?

____ In the motivation to using the on-off scheme, mention that there is an advantage in setting a constant trasnmit power by the Tx, in this case constant envelope communication with efficient power amplifier is possible.  	


_In outage analysis sections, mention the effect of the factors rho and bets.. rho scales the threshold SNR so a higher threshold is obtained. beta scales the average harvested energy down.

Mention that these BE and On-OFF schemes have been studied for a rayleigh fading channels in my conference papers, and that this paper extends them to Nakagami-m fading which is more general type that covers many theoretical channel models and empirircal channels too. also we study different effects and provide closed-form expressions for the outage probability

_Introduction: From http://berc.berkeley.edu/storage-wars-batteries-vs-supercapacitors/
 Energy storage technologies have the potential to offset the intermittency problem of renewable energy sources by storing the generated intermittent energy and then making it accessible upon demand. 
 
 --Introduction. Storage therefore allows to regulate and control the transmit power from the EH node instead of leaving it to fluctuate randomly just as the randomly fluctuating EH source. 
___System model. In fact it is in general OK to transmit all the DL power on a ingle frequency (i.e., zero bandwidth). However, usually the power limitations by FCC is specified by a power spectral density Mask, i.e., there is a limit on the power trasmitted on each frequency. Hence, if we want to transmit with a total power of P, we might be forced to distribute the power over a frequency band to fullfill the PSD requirements. If however, the total effective isotropic radiated power Pdl*Gt is still below the maximum allowed PSD, then all the power can be placed in a single frequency. Otherwise, the power can be distributed on the minimum bandwidth needed. We note that in any case, the transmit power by the EH node is limited to M, so increasing the DL power (and therefore the average harvested energy) beyond a certain value does not improve the outage probability performance. 
If we use TDD, then we can use the same bandwidth used by the information channel. If we use FDD, i.e., EH and transmission take place concurrently on two different bands, then we just use the least bandwith needed for transmitting all the power we want.

--In first corollary, mention that considering continuous state  is better in that we need to invert an mxm matrix, where realistic values of m are small, and even whenn m represents the number of antennas, they are small compared to inverting matrices of size LxL where L is the number of battery levels which has to be large enough for accurate results. Hence, we get th exact distribution with less complicated matrix inversion. 

---Motivation of closed-form expressions and integral equations
Remark: We note that if a transmission policy is based on the amount of the stored energy, then getting the limiting distribution of the stored energy is essential to analyze almost any performance measure of the system. To this end, for a given transmission policy, the limiting energy distribution can be obtained in two steps. First, the integral equation of the limiting distribution can be formulated for any general i.i.d. EH process. Second, given the statistics of the EH process, the limiting energy distribution can then be obtained by solving the integral equations.

==> figures/g_x_stripes <==
<?xml version="1.1" encoding="windows-1252"?>
<svg xmlns="http://www.w3.org/2000/svg"
    xmlns:latexdraw="http://latexdraw.sourceforge.net/namespaces/latexdraw"
    version="1.1" baseProfile="full">
    <g>
        <g latexdraw:type="joinedLines" id="id1175334650">
            <polyline points="205.0,660.0 1020.0,660.0 1020.0,660.0 "
                stroke-width="2.0" stroke="black" fill="none"
                latexdraw:rotationAngle="0.0" marker-end="url(#arrow1-1175334650)"/>
        </g>
        <g latexdraw:type="joinedLines" id="id668292305">
            <polyline points="1000.0,670.0 1000.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id995814675">
            <polyline points="900.0,670.0 900.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id493824576">
            <polyline points="205.0,670.0 205.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id604028529">
            <polyline points="700.0,670.0 700.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id1624141986">
            <polyline points="600.0,670.0 600.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id950930005">
            <polyline points="250.0,670.0 250.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id1900587077">
            <polyline points="350.0,670.0 350.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="joinedLines" id="id1163687944">
            <polyline points="450.0,670.0 450.0,650.0 "
                stroke-width="2.0" stroke="black" latexdraw:rotationAngle="0.0"/>
        </g>
        <g latexdraw:type="text" id="id1845887086" fill="black" latexdraw:position="bl">
            <text x="794.4117647058821" y="644.705882352941">$\ldots$</text>
        </g>
        <g latexdraw:type="text" id="id781788948" fill="black" latexdraw:position="bl">
            <text x="989.1176470588232" y="688.2352941176468">$K$</text>
        </g>
        <g latexdraw:type="text" id="id1357070451" fill="black" latexdraw:position="bl">
            <text x="875.2941176470586" y="690.2941176470586">$K-M$</text>
        </g>
        <g latexdraw:type="text" id="id80485950" fill="black" latexdraw:position="bl">
            <text x="672.0588235294115" y="692.3529411764704">$K-nM$</text>
        </g>
        <g latexdraw:type="text" id="id509425681" fill="black" latexdraw:position="bl">
            <text x="552.0588235294116" y="692.3529411764704">$K\!\!-\!(\!n\!+\!1\!)M$</text>
        </g>
        <g latexdraw:type="text" id="id1841760490" fill="black" latexdraw:position="bl">
            <text x="196.76470588235287" y="687.3529411764704">$0$</text>
        </g>
        <g latexdraw:type="text" id="id2096120676" fill="black" latexdraw:position="bl">
            <text x="222.0588235294117" y="689.4117647058821">$K\!\!\!-\!\!lM\!\!=\!\!\Delta$</text>
        </g>
        <g latexdraw:type="text" id="id776203216" fill="black" latexdraw:position="bl">
            <text x="312.05882352941165" y="694.4117647058821">$K\!\!-\!(\!l\!-\!1\!)M$</text>
        </g>
        <g latexdraw:type="text" id="id507635810" fill="black" latexdraw:position="bl">
            <text x="417.05882352941165" y="694.4117647058821">$K\!\!-\!(\!l\!-\!2\!)M$</text>
        </g>
        <g latexdraw:type="text" id="id1329624781" fill="black" latexdraw:position="bl">
            <text x="514.4117647058821" y="644.705882352941">$\ldots$</text>
        </g>
        <g latexdraw:type="text" id="id441722843" fill="black" latexdraw:position="bl">
            <text x="938.2352941176468" y="649.4117647058822">$g_0(x)$</text>
        </g>
        <g latexdraw:type="text" id="id549994020" fill="black" latexdraw:position="bl">
            <text x="638.2352941176468" y="649.4117647058822">$g_n(x)$</text>
        </g>
        <g latexdraw:type="text" id="id1714389821" fill="black" latexdraw:position="bl">
            <text x="378.23529411764684" y="649.4117647058822">$g_{l\!-\!2}(x)$</text>
        </g>
        <g latexdraw:type="text" id="id462782890" fill="black" latexdraw:position="bl">
            <text x="273.23529411764684" y="649.4117647058822">$g_{l\!-\!1}(x)$</text>
        </g>
        <g latexdraw:type="text" id="id1036741181" fill="black" latexdraw:position="bl">
            <text x="213.23529411764684" y="649.4117647058822">$g_l(x)$</text>
        </g>
    </g>
    <defs>
        <marker overflow="visible" orient="auto" id="arrow1-1175334650">
            <path
                d="M 0.0 0.0 L -4.652083333333334 1.6614583333333335 L -4.652083333333334 0.0 L -4.652083333333334 -1.6614583333333335 z "
                latexdraw:arrSizeNum="2.0" fill="black"/>
        </marker>
    </defs>
    <metadata>
        <latexdraw:metadata>
            <latexdraw:latexIncludes/>
            <latexdraw:displayXScale>true</latexdraw:displayXScale>
            <latexdraw:displayYScale>true</latexdraw:displayYScale>
            <latexdraw:unit>CM</latexdraw:unit>
            <latexdraw:zoom>1.7000000000000006</latexdraw:zoom>
            <latexdraw:magneticGridStyle>STANDARD</latexdraw:magneticGridStyle>
            <latexdraw:gridGap>20</latexdraw:gridGap>
            <latexdraw:magneticGrid>true</latexdraw:magneticGrid>
            <latexdraw:version>3.3.4</latexdraw:version>
            <latexdraw:size>
                <latexdraw:width>1920</latexdraw:width>
                <latexdraw:height>1176</latexdraw:height>
            </latexdraw:size>
            <latexdraw:position>
                <latexdraw:x>0.0</latexdraw:x>
                <latexdraw:y>0.0</latexdraw:y>
            </latexdraw:position>
        </latexdraw:metadata>
    </metadata>
</svg>


==> proof_OO_stationary_dist_infinite_existence_and_uniqueness.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{theo:stationary_dist_infinite} (Existence and Uniqueness of a Limiting Energy Distribution for an Infinite-Size Buffer with the On-Off policy)}
\label{app:stationary_dist_infinite_OO}
In the double service rate model by Gaver and Miller c.f. Remark \ref{remark:equivalence_onoff_to_Millers_model}, if the (average service time $\times$ arrival rate $<$ release rate $r_2$), then the existence and the uniqueness of the limiting distribution for the waiting time is guaranteed, see \cite[p.112]{Gaver_Miller_1962}. In our model, this condition translates to $\E[X]<M$. This completes the proof.
%%%%%%%%%%%%%%%%%%%d%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
